A Posterior Error Estimator for Mixed Interior Penalty Discontinuous Galerkin Finite Element Method for the H(curl)-Elliptic Problems

In this paper, we design the first residual type a posteriori error estimator for mixed interior penalty discontinuous Galerkin method for the H(curl)-elliptic problems. Then we prove that our residual based a posteriori error indicator is both reliable and efficient. At last, we present some numerical experiments to validate the performance of the indicator within an adaptive mesh refinement procedure.

==> Coverletter/coverletter.tex <==
 We would like to submit the enclosed manuscript entitled “A Posterior Error Estimator for Mixed Interior Penalty Discontinuous Galerkin Finite Element Method for the  $\boldsymbol{H}(\mathrm{curl})$-Elliptic Problems” by Ming Tang, Xiaoqing Xing,  and Liuqiang Zhong, which we wish to be considered for publication in “Journal of Computational and Applied Mathematics”.  We believe that this manuscript will make it interesting to general readers of this journal. 
 All authors have read and approved this version of the article, and due care has been taken to ensure the integrity of the work. No part of this paper has been published or submitted elsewhere. No conflict of interest exists in the submission of this manuscript.
We hope you will give favorable consideration to our manuscript and find the article acceptable for publication in your journal. Please contact me should I be of further assistance. Thank you very much for your help. I am looking forward to hearing from you.
